Towards Fine-Grained Video Question Answering

In the rapidly evolving domain of video understanding, Video Question Answering (VideoQA) remains a focal point. However, existing datasets exhibit gaps in temporal and spatial granularity, which consequently limits the capabilities of existing VideoQA methods. This paper introduces the Multi-Object Multi-Actor Question Answering (MOMA-QA) dataset, which is designed to address these shortcomings by emphasizing temporal localization, spatial relationship reasoning, and entity-centric queries. With ground truth scene graphs and temporal interval annotations, MOMA-QA is ideal for developing models for fine-grained video understanding. Furthermore, we present a novel video-language model, SGVLM, which incorporates a scene graph predictor, an efficient frame retriever, and a pre-trained large language model for temporal localization and fine-grained relationship understanding. Evaluations on MOMA-QA and other public datasets demonstrate the superior performance of our model, setting new benchmarks for VideoQA.

==> deprecated/deprecated.tex <==
% Introduction

In light of the rapid progress in the realm of large language models (LLMs), we have witnessed a significant expansion in the scale of foundational language models. Contemporary LLMs are trained on an astonishing scale, reaching up to trillions of tokens \cite{hoffmann2022empirical, touvron2023llama}. This scale surpasses image-text datasets by orders of magnitude \cite{schuhmann2022laion}. The extensive training data at their disposal empowers these models with enhanced reasoning capabilities \cite{qiao2022reasoning}, a competency that is indispensable for the Visual QA task. Consequently, \textit{large language model-based (LLM-based)} vision models have consistently outperformed their counterparts in numerous image QA benchmarks \cite{alayrac2022flamingo, blip2}. Nonetheless, the Video QA domain, characterized by the intricate spatial-temporal dynamics of videos, presents unique challenges \cite{xiao2020visual, zhong2022video}. As a result, VLMs that excel in image-based tasks don't always guarantee parallel success in video contexts due to their limited length of input. Works have been proposed to leverage LLM itself to filter the relevant frames, but such method is computationally expensive and offers limited gains \cite{yu2023self}.

% TODO: The part below is too long

% Part: QA on temporal localization

As important as it is for models to infer actions or activities within a video, it is equally important for them to comprehend when these activities occur in relation to particular frames. Foundational Video QA datasets like MSRVTT-QA \cite{xu2017video} lack focus on temporal grounding. Around 33.4\% of its questions can be boiled down to the inquiry, "What is [someone] doing?" These types of questions primarily drive models toward video classification tasks and do not require the model to tie its responses to particular timeframes or sequences in the video. While more recent works like TVQA+ and TGIF-QA \cite{lei2019tvqa+, jang2017tgif} do put focus on temporal reasonings, their source videos are short enough so that a uniform sampling of a few frames guarantees good performance \cite{yu2023self}.

The consequences of this unbalanced emphasis are significant. Their performance deteriorates in scenarios that require long-form video comprehension, such as deciphering the complexities of a movie plot or conducting continuous surveillance analyses. Due to the limited purview of the datasets, the models lack the granularity necessary for such intricate analysis.

% Part: QA on spatial relationship

Second, the spatial relationship comprehension of a video's elements is fundamental to a comprehensive Video QA system. It involves recognizing the relative placement and interaction of objects and entities within the visual field. Regrettably, even datasets that boast their granularity provide models with limited opportunities to refine their spatial understanding. As an example, within the ActivityNet-QA dataset \cite{yu2019activitynet}, only 10\% of its queries involve questions with spatial relationships. Given that spatial dynamics form the foundation of a number of actual video scenarios, this underrepresentation is concerning. Models trained on these datasets may be proficient at recognizing individual objects or activities but may struggle to comprehend their interplay.
